Investigating the Role of Feed-Forward Networks in Transformers Using Parallel Attention and Feed-Forward Net Design

This paper investigates the key role of Feed-Forward Networks (FFNs) in transformer models by utilizing the Parallel Attention and Feed-Forward Net Design (PAF) architecture, and comparing it to their Series Attention and Feed-Forward Net Design (SAF) counterparts. Central to the effectiveness of PAF are two main assumptions regarding the FFN block and the attention block within a layer: 1) the primary function of the FFN block is to maintain isotropy among token embeddings and prevent their degeneration, and 2) the residual norm computed in the attention block is substantially smaller than the input token embedding norm. To empirically validate these assumptions, we train PAF variants of two large language models (RoBERTa-large and bert-large-uncased). Our results demonstrate that both assumptions hold true in the PAF design. This study contributes to a deeper understanding of the roles and interactions between FFNs and self-attention mechanisms in transformer architectures.

==> figures/iso.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.4]{images/iso.png}
    \caption{hello}
    \label{fig:iso}
\end{figure*}

==> figures/resnorm.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[scale=0.5]{images/resnorm.png}
    \caption{On the left is the standard \longsaf (\safns) for transformers models. On the right is our proposed \longname (\namens) design for transformer models.}
    \label{fig:pfa}
\end{figure*}

==> sections/experiments.tex <==
\input{tables/glue}

\subsection{Pre-training of \name models}

To test the efficacy of \name design, we pre-trained two large language models RoBERTa-Large \cite{roberta} and Bert-Large-Uncased \cite{bert} on English Wikipedia and BooksCorpus \citep{bookcorpus}.
Both models are 24 layer models and widely used in various NLP applications.
We initialize the parameters for \name models using their \saf variants and follow guidelines for learning rate, optimizer, and loss functions\footnote{\url{https://tinyurl.com/495vfeh9}}.
Each model is trained on four NVIDIA RTX A6000 gpus for a total of 72 hours.

\subsubsection*{Fine-tuning details on the GLUE benchmark}
We tested the effectiveness of the pre-trained \name variants of RoBERTa-Large and Bert-Large-Uncased, we finetune both models on the General Language Understanding Evaluation (GLUE) benchmark \cite{glue}.
GLUE benchmark assesses various NLP tasks that range textual entailment (MNLI, QNLI), paraphrase detection (MRPC, QQP), sentence similarity (STS-B) and sentiment analysis (SST-2).
The GLUE benchmark is a widely recognized evaluation standard for NLP models and provides a comprehensive evaluation of the performance of NLP models.
Each task in GLUE is trained using the recommended\footnote{\url{https://tinyurl.com/26xd6js6}} hyperparameter choices which include learning rate, batch size, warmup steps, and optimizer settings on a single Quadro RTX 8000 GPU for five random seeds.
We exclude the two smallest datasets of the GLUE benchmark - CoLA and RTE because of the high instability and variance in their fine-tuning \citep{unstablebert}.

\subsection*{\name evaluation on GLUE benchmark}
As can be seen in table \ref{tab:glue}, \name variants of both RoBERTa-Large and Bert-Large-Uncased perform nearly identically to their \saf equivalents.
The gap for RoBERTa-Large is slightly less smaller than Bert-Large-Uncased ($0.6\%$ vs $0.1\%$) which can be attributed to eight times smaller size of data used to train the \name variant of RoBERTa-Large.
RoBERTa models were trained on 160GB size dataset, however we only use 20 GB wikipedia and BooksCorpus dataset.


==> sections/safekeep_writing.tex <==
% One of the important functions of the feed forward block is keep the vectors apart.
% Residuals is very small compared to the main embedding.
% So, to push apart the embeddings, we do not need the residual.
% Hence, we can parallelize.

% Arguments 1: FFN block's most important function is to maintain a level of optimal anisotropy in higher layers.

% It is easy to show that one of the functions of FFN block is to maintain a level of optimal anisotropy with the plots.

% But it is tricky to show that it is the most important.
% To show that 1) we can show $x$ and $x'$ have similar performance 2) train a network without FFN blocks and show that models without FFN blocks works almost similar, but the anisotropic representations are advantageous.

% Arguments 2: If the function of FFN block is to spread out the vectors, the spread can be also be done on $x$, rather than $x +\delta x$ if $ x +\delta x \sim x $. 
% Need to show $\norm{x} >> \norm{\delta x}$, $\norm{x'} >> \norm{\delta x'}$, easy to show.
